Predicting IPv4 Services Across All Ports

Internet-wide scanning is commonly used to understand the topology and security of the Internet. However, IPv4 Internet scans have been limited to scanning only a subset of services -- exhaustively scanning all IPv4 services is too costly and no existing bandwidth-saving frameworks are designed to scan IPv4 addresses across all ports. In this work we introduce GPS, a system that efficiently discovers Internet services across all ports. GPS runs a predictive framework that learns from extremely small sample sizes and is highly parallelizable, allowing it to quickly find patterns between services across all 65K ports and a myriad of features. GPS computes service predictions in 13 minutes (four orders of magnitude faster than prior work) and finds 92.5% of services across all ports with 131x less bandwidth, and 204x more precision, compared to exhaustive scanning. GPS is the first work to show that, given at least two responsive IP addresses on a port to train from, predicting the majority of services across all ports is possible and practical.

==> scraps.tex <==

\begin{figure}[h!]
  %\centering
  \includegraphics[width=0.5\textwidth]{figures/all24_dist_predict.pdf}
 \caption{\textbf{Limitations of Feature Correlations}---%
 }
  \label{fig:corr_predict}
\end{figure}


%Figure~\ref{fig:censys_net_predict} illustrates the fraction of normalized services and all services that could theoretically be found using a randomly sampled 1\% IPv4 ``seed set,'' (i.e., there is at least one service responding on the same port in the same sub-network in the 1\% seed set).  Note we choose a 1\% IPv4 sub-sample across all 65K ports as an approximate available large sub-sample, as it takes approximately 1~month to scan at a rate that minimizes packet-drop and denial-of-service (i.e., 50~MB/s).  Only 19\% of normalized services could theoretically be found using a 1\% seed set if using a /11 subnetwork size, compared to 96\% of all services. 

%\textbf{Host Discovery} While network patterns do not suffice to find the majority of normalized services, they are more helpful at finding hosts that respond on an uncommon ports. Figure~\ref{fig:censys_net_predict} shows that the slim majority of normalized hosts can be found when relying spatial patterns. This indicates that spatial patterns are more useful at finding the set of initial hosts to find other uncommon services on. \todo{forward ref}


We define the ``predictability'' of a port, using a particular pattern as prior knowledge (e.g., sub-network) to be the sum of all probabilities of discovering the IP using the pattern with the highest hitrate (Equation~\ref{eq:predictability}) 
\begin{equation} \label{eq:predictability}
\mbox{predictability = } \frac{\sum_{i=1}^{\# IPs} \mbox{MAX(}\frac{\mbox{\# IPs responding on target port }}{\mbox{\# IPs exhibiting Pattern}}\mbox{)}}{\mbox{\# IPs on target port}}
\end{equation}

The sum of all normalized services that can be found just by using all 24~features is 384/2000 ports.





\todo{RE: I wonder if we need to talk about recommendation systems at all. As is, it is really hard to know what you did and whether some alternative way of setting this up wouldn't work. Maybe you can get to the main challenges when discussing the prior work? If you decide to keep this, it seems odd that you have the part you did within prior work.}
\textbf{Recommendation System}
Prior work's use of machine learning, but lack of a scalable solution across all 65K ports, inspire us to apply a machine learning framework that has been successful at scaling to multi-dimensional problems in non-networking applications: recommendation systems. Proprietary recommendation systems have been successful at recommending millions of potential items to millions of potential users at Netflix~\cite{gomez2015netflix}, Spotify~\cite{mcinerney2018explore}, and Amazon~\cite{ma2020temporal}, thus inspiring us to apply the model to recommend potential ports to IPs. 
However, we explore over 30~different open source recommendation models~\cite{recMic} and find that feature ingestion for current open source Recommendation Systems is not suitable for Intelligent Scanning; Recommendation System allow features to be assigned to users (i.e., IPs) and/or items (i.e., ports), but do not directly allow for features to be assigned to IP,Port tuples (i.e., their interaction). This means that features tied to particular services on a host (e.g., TLS cert on port 400) cannot easily be represented.
Nonetheless, we implement a collaborative-filtering model using LightFM~\cite{kula2015metadata} 
%\todo{regardless, we implement using LightFM...}


%%%%%%%%%%%%%%
\system's ability to predict services is  directly dependent on the size of the seed scan (Section~\ref{sub:sub:sec:seed}), as \system relies on the seed scan to learn service-presence patterns.
For any potential system that relies on seeing a service-presence pattern to help predict other service (e.g., machine learning classifiers) the size of a seed set presents an inevitable theoretical limitation. 




To understand the theoretical limitation of predicting services when relying on a seed set---and how \system's performance compares---we plot in Figure~\ref{fig:fund_predict} the theoretical maximum fraction of normalized services that can be found using a 1\% uniformly-random IPv4 seed scan, relative to a scanning step size. 


We calculate the theoretical predictable-by-network-patterns maximum by filtering for all services that appear on a host that shares at least one same open port in the same sub-network (dependent on the scanning step size) in the seed set (i.e., the pattern is present in the seed set). In other words, if an open port is present in a sub-network at least once in the seed scan, this opens the possibility for the port to be exhaustively scanned in the sub-network, thereby discovering the host, and further opening the possibility that all other services on the host can be discovered (e.g., through the use of port correlations). 
However, if the seed set has never seen any of a host's open ports in the same subnetwork before, no predictive system relying on sub-network patterns will be able to informatively predict those ports without attempting to randomly ``guess'' (therefore costing more probes). 

Across all scanning step sizes, \system consistently finds roughly 82\% of the theoretical maximum fraction of normalized services. For example, at a scanning step size of /0 (i.e., requiring that at least one port on a host has been seen anywhere in the seed scan), 100\% of hosts can \textit{theoretically} be found and \system finds 82\% of all normalized hosts. At a scanning step size of /20, only 55\% (1098/2000) of normalized services can theoretically be discovered and \system finds 82\% of such hosts. 

While patterns dominate services, random configurations of hosts will always present a limitation for predicting services (Section~\ref{sub:sub:sec:net_patterns}).
\system does not find all possible normalized services primarily because 
\system is designed to scan two categories of service space:  services that are predictable and services that help predict other services (i.e., the priors and posteriors of Equations~\ref{eq:l4}--\ref{eq:l4_l7_host} that maximize the probability of a service being found). By scanning only these two categories, \system is able to perform better than exhaustive random probing and therefore conserve bandwidth.
However, services that are not predictable or do not help predict other services---and services that follow a pattern not seen in the seed scan---will not be attempted to be found by \system, as it will require more randomized probing. 

\todo{Going to compare ``predictability'' of things system gets vs things system misses. }

When using \system with a /0 scanning step size and 1\% seed scan, 62\% of normalized services that \system cannot find live on hosts that only respond on one port.
Consequently, these services can only be found by exhaustively scanning their sub-network on the single port they respond on---as no other service on the host is available to provide a ``hint'' that the other port may be open.
Of the remaining 38\% of services that \system cannot find and that exist on hosts that respond on more than one port, 98\% of such services appear together with ports that---together---the 1\% seed scan has never seen before (e.g., host A has ports 81 and 999 open---a pattern never seen in the 1\% seed set). As a result, there is no way for \system to have known that one of the host's open ports was predictive of the other.

We leave \system's ability to precisely infer new patterns (e.g., perhaps by using deep learning) as future work. 
%97\% respond on two or less ports.



We hypothesize that \system can best achieve its goal by taking advantage of a myriad of features, including transport-layer features, port correlations, and application-layer features (Section~\ref{sub:predictability}).


\begin{figure}[h!]
  %\centering
  \includegraphics[width=0.5\textwidth]{figures/networkPattern_censys_1p_skips.pdf}
 \caption{\textbf{Limitations of Network Patterns}---Censys 1p->100p%
 }
  \label{fig:fund_predict}
\end{figure}

the sum of all probabilities of discovering the IP using the pattern with the highest hitrate (Equation~\ref{eq:predictability}) 
\begin{equation} \label{eq:predictability}
\mbox{predictability = } \frac{\sum_{i=1}^{\# IPs} \mbox{MAX(}\frac{\mbox{\# IPs responding on target port }}{\mbox{\# IPs exhibiting Pattern}} * \frac{\mbox{\# IPs exhibiting Pattern}}{\mbox{\# IPs on Target Port}} \mbox{)}}{\mbox{\# IPs on target port}}
\end{equation}


When finding the first 5\% of normalized services, \system saves \textit{four orders of magnitude} of bandwidth (i.e., finds the services 4~orders of magnitude faster)  compared to exhaustive/random scanning 
This means that, when scanning at 1Gb/s, services across over 3K ports can be found in less than 1~minute. 
\system's precision, and thus speed, decays as it finds more normalized services, as the predictability of services being scanned also decays.  
For example, \system saves three orders of magnitude compared to exhaustive/random scanning when finding the first 25\% of normalized services.
